Efficient Centroid-Linkage Clustering

We give an efficient algorithm for Centroid-Linkage Hierarchical Agglomerative Clustering (HAC), which computes a $c$-approximate clustering in roughly $n^{1+O(1/c^2)}$ time. We obtain our result by combining a new Centroid-Linkage HAC algorithm with a novel fully dynamic data structure for nearest neighbor search which works under adaptive updates. We also evaluate our algorithm empirically. By leveraging a state-of-the-art nearest-neighbor search library, we obtain a fast and accurate Centroid-Linkage HAC algorithm. Compared to an existing state-of-the-art exact baseline, our implementation maintains the clustering quality while delivering up to a $36\times$ speedup due to performing fewer distance comparisons.

==> A1_centroidClusterDefinition.tex <==
\section{Cluster-Centric Definition of Centroid-Linkage HAC}\label{sec:centroidClusterDefinition}

We formally define Centroid-Linkage HAC in a cluster-centric way. For a set of points $X \subset \R^d$, we define $\cent{X}$ to be the centroid of $X$ as below.

\begin{definition}[Centroid] \label{def:centroid}
    Given a set of points $X \subset \R^d$, the centroid of $X$ is the point $x \in \R^d$ whose $i$th coordinate is 
    \begin{align*}
        x[i] = \sum_{y \in X} \frac{y[i]}{|X|}.
    \end{align*}
\end{definition}

Centroid HAC uses distance between centroids as a linkage function. That is, for clusters $X$ and $Y$,
\begin{align*}
    \mathcal{L}(X,Y) = \dist{\cent{X}}{\cent{Y}}.
\end{align*}
$c$-approximate Centroid-Linkage HAC is defined as follows. We are given input points $P \subset \R^d$. First, initialize a set of active clusters $\mcC = \{ \{p\} \}_{p \in P}$.  Then, until $|\mcC| = 1$ we do the following: let $\hat{X}, \hat{Y} \in \mcC$ be a pair of active clusters satisfying
\begin{align*}
    \mathcal{L}(\hat{X}, \hat{Y}) \leq c \cdot \min_{X, Y \in \mcC} \mathcal{L}(X, Y)
\end{align*}
where the $\min$ is taken over distinct pairs; merge $\hat{X}$ and $\hat{Y}$ by removing them from $\mcC$ and adding $\hat{X} \cup \hat{Y}$ to $\mcC$. (Non-approximate) Centroid-Linkage HAC is just the above with $c = 1$.

==> A3_proofs-ann.tex <==
% \section{Proofs from \Cref{sec:ann}}

% \covnet*

% \begin{proof}
    
% \end{proof}



==> A4_proofs-centroidHAC.tex <==
\section{Proofs from \Cref{sec:Centroid_Hac}}

We now prove that \Cref{alg:SIMPLE_HAC} gives a $(c(1+\epsilon))$-approximate HAC where $c$ is the approximation value inherited from the approximate nearest neighbor data structure. Note that a smaller $\epsilon$ will give a more accurate HAC but will increase the runtime of the algorithm.

\begin{lemma} \label{lem:SIMPLE_HAC_CORRECTNESS}
   Algorithm \ref{alg:SIMPLE_HAC} gives a $c(1+\epsilon)$-approximate Centroid-Linkage HAC.
\end{lemma}

\begin{proof}
    The idea of the proof is to observe that one of the two endpoints of the closest pair will always store an approximate of the minimum distance in $Q$. In that spirit, suppose that right before a centroid is dequeued, the shortest distance between active centroids is $l_\opt$. Then there must exist active centroids $x_1$ and $x_2$ such that $D(x_1, x_2) = l_\opt$. Assume without loss of generality that $x_1$ was queued before $x_2$ and $x_2$ was queued with distance $l_2$. Then, when $x_2$ was queued, $x_1$ was active so $l_2 \leq c \cdot l_\opt$.

    Thus, when a centroid, $x$, is dequeued, its distance $l_x$ obeys the inequality 
    $$l_x \leq l_2 \leq c \cdot l_\opt.$$ Then, if $x$ is merged during the while loop, it is merged with a centroid of distance at most $$(1+\epsilon) l_x \leq c (1 + \epsilon) l_\opt$$ as desired. If a centriod gets merged without being dequeued, that means it merged with another identical centroid which is consistent with $1$-approximate HAC.
\end{proof}

We now prove the runtime of the algorithm. Say that the maximum pairwise distance between points in $P$ is $\Delta$ and the minimum is $\delta$. We make the following observations about the geometry of the centriods throughout the runtime of \cref{alg:SIMPLE_HAC}.

\begin{observation} \label{obs:contained_in_ball}
    Consider any point $p \in P$. Throughout the runtime of \cref{alg:SIMPLE_HAC}, the distance from any centroid to $p$ is at most $\Delta$.
\end{observation}

\begin{proof}
    Consider a cluster $Q \subseteq P$. Since for each $q \in Q$ we have $D(p,q) \leq \Delta$, it follows that $D(p,\text{cent}(Q)) \leq \Delta$.
\end{proof}

\begin{observation} \label{obs:few_close_points}
    When running \cref{alg:SIMPLE_HAC}, at any point in time there can only ever be a single centroid queued with distance less than $\delta$.
\end{observation}

\begin{proof}
    Initially, every centroid is queued with distance at least $\delta$. Thus, if a centroid is ever queued with a smaller distance it will immediately be dequeued and merged.
\end{proof}

\begin{lemma} \label{lem:SIMPLE_HAC_RUNTIME}
   Algorithm \ref{alg:SIMPLE_HAC} runs in time $O( n \cdot T_I + n \cdot T_D + n \cdot T_Q \cdot \log_{1+\epsilon} (\frac{2 \Delta}{\delta}) + n \log (n) \log_{1+\epsilon} (\frac{2 \Delta}{\delta}))$.
\end{lemma}

\begin{proof}
    The idea of the proof is that each time we dequeue a centroid we either merge it or we increase the distance associated with it by a multiplicative factor of $1+\eps$ which can only happen $\log_{1 + \epsilon}(2 \Delta / \delta)$ times for each of our $O(n)$-many centroids.

    Each centroid is inserted into $\N$ at most once, either during the initial construction or in \cref{alg:MERGE}, and deleted at most once. Since there are $2n - 1$ centroids throughout the runtime, the total time spent on updates to $\N$ is $O(n \cdot T_I + n \cdot T_D)$.

    At any given point during the algorithm, a centroid can be in $Q$ at most once. Since only $2n - 1$ centroids are ever created, there are at most $2n - 1$ elements in $Q$ at any time. Thus, a single queue or dequeue operation takes $O(\log(n))$ time. In the initial for loop we queue $n$ elements to $Q$ and make $n$ queries to $\N$ taking time $O(n \log(n) + n \cdot T_Q)$. Each time algorithm \ref{alg:MERGE} gets called it queues one element to $Q$ and makes up to $4$ updates to $C$. Since \cref{alg:MERGE} is called at most $n - 1$ times, the total time spent on merges, not including updates to $\N$, is $O(n \cdot T_Q + n \log(n))$.

    Lastly, we consider how many times a centroid $x$ can be dequeued on \cref{line:dequeue}. Suppose $x$ is queued with distance $l_i$ the $i$th time it is queued. If $l_1 < \delta$ then by \cref{obs:few_close_points}, $x$ will be immediately dequeued and merged so $x$ is only queued once. Thus, we assume $l_1 \geq \delta$. If $x$ is dequeued with distance $l_i$ then either $x$ is merged and will not be queued again or it is queued again with distance $$l_{i+1} > (1 + \epsilon) l_i > (1 + \epsilon)^i l_1.$$ Since $l_1 \geq \delta$ by assumption and $l_i \leq 2 \Delta$ for all $i \geq 1$ by \cref{obs:contained_in_ball}, it follows that $x$ can only be queued, and therefore dequeued, $\log_{1 + \epsilon} (\frac{2 \Delta}{\delta})$ times. Each time, not including merges, there can be one dequeue from $Q$, one queue to $Q$, and one query to $\N$. Since there are $2n - 1$ centroids created by the algorithm, the while loop (not including merges) runs in time $O(n \log (n) \log_{1+\epsilon} (\frac{2 \Delta}{\delta}) + n \cdot T_Q \cdot \log_{1+\epsilon} (\frac{2 \Delta}{\delta}))$.
\end{proof}

Combining the previous two lemmas together we get the following.

\hacReduction*
\begin{proof}
    By \cref{lem:SIMPLE_HAC_CORRECTNESS} and \cref{lem:SIMPLE_HAC_RUNTIME} we get that \cref{alg:SIMPLE_HAC} gives $c(1 + \epsilon)$-approximate HAC in time $O( n \cdot T_I + n \cdot T_D + n \cdot T_Q \cdot \log_{1+\epsilon} (\frac{2 \Delta}{\delta}) + n \log (n) \log_{1+\epsilon} (\frac{2 \Delta}{\delta}))$. It is only left to show that $\log_{1+\epsilon} (\frac{2 \Delta}{\delta}) \leq \polylog (n)$. Changing the base of the logarithm we get

    $$\log_{1+\epsilon} \Big(\frac{2 \Delta}{\delta}\Big) = \frac{\log(\frac{2 \Delta}{\delta})}{\log (1 + \epsilon)}.$$

    We have that $\log(\frac{2 \Delta}{\delta}) \leq \polylog(n)$ by the assumption that $\frac{\Delta}{\delta} \leq \poly(n)$. By the inequality $\log(1+x) \geq \frac{x}{1 + x}$ for all $x > -1$ we get that if $\epsilon \leq 1$
    \begin{align*}
        \frac{1}{\log(1 + \epsilon)} \leq \frac{1 + \epsilon}{\epsilon} \leq \frac{2}{\epsilon} =  O\Big(\frac{1}{\epsilon}\Big) \leq \polylog(n)
    \end{align*}
    where the final inequality comes from the assumption that $\frac{1}{\epsilon} \leq \polylog(n)$. If $\epsilon > 1$ then
    \begin{align*}
        \frac{1}{\log(1 + \epsilon)} \leq \frac{1}{\log(2)} \leq \polylog(n).
    \end{align*}
    Combining the above inequalities and the above-stated runtime gives our final runtime.
\end{proof}


We use \cref{thm:general_hac} with our results from \cref{sec:ann} to get our main result. First we prove the following lemma which says that our ANNS that includes an additive term functions as a purely multiplicative ANNS for our algorithm.

\begin{lemma} \label{lem:mult_ann}
        For any $\lambda \in (1,c)$, if $\N$ is a $\Big(\frac{c}{\lambda}, \frac{\delta (\lambda - 1)}{(1+c) \lambda}\Big)$-approximate NNS data structure that works for adaptive updates then $\N$ is a $c$-approximate NNS data structure for all queries in \cref{alg:SIMPLE_HAC}.
    \end{lemma}

    \begin{proof}
        Let $C$ be the set of active centroids at the time any given query takes place. We will say a point $x$ is close to the set $C$ if $D(x,C) < \frac{\delta}{c}$. We show that if $x$ is not close to $C$, then $\N^{\text{query}}(x,x) = y$ will give us the multiplicative result we desire:

        \begin{align}\label{eq:not_close}
            \nonumber  D(x, y) &\leq \frac{c}{\lambda} D(x,C) + \frac{\delta (\lambda - 1)}{(1+c) \lambda}\\
            \nonumber &\leq \frac{c}{\lambda} D(x,C) + \frac{\delta}{c} (\lambda - 1)\\
            \nonumber &\leq \frac{c}{\lambda} D(x,C) + D(x,C) (\lambda - 1)\\
            \nonumber &< \frac{c}{\lambda} D(x,C) + D(x,C) \frac{c (\lambda - 1)}{\lambda}\\ \nonumber
            \nonumber &\leq c \cdot D(x,C) \Big(\frac{1}{\lambda} + \frac{\lambda - 1}{\lambda}\Big)\\ 
            &\leq c \cdot D(x,C).
        \end{align}

        We now prove the lemma by induction. The base case is the set of neighbors calculated for the initial set of points $P$. Each $p \in P$ is not close to $C \setminus p$ so by \cref{eq:not_close}, 
        
        $$D(p,\N^{\text{query}}(p,p)) < c \cdot D(p, C \setminus p)$$
        
        as desired. Now for the induction step, consider some query for a centroid $x$ that has just been dequeued. For $x,y \in C$, say $y$ is a $c$-approximate nearest neighbor of $x$ if $\dist{x}{y} \leq c \cdot \dist{x}{C \setminus x}$. Assume by induction that all queries up to this point have returned $c$-approximate nearest neighbors. We know by \cref{obs:few_close_points} and the inductive hypothesis that either no points are close to $C$ or $x$ is the lone point that is close to $C$. In the former case, $\N$ returns a $c$-approximate nearest neighbor by \cref{eq:not_close}. Now consider the latter case. Let $y$ be a centroid such that $\dist{x}{y} > c \cdot \dist{x}{C \setminus x}$. We will show that $\N^{\text{query}}(x,x) \neq y$.

        Define $L = \dist{x}{y} + \dist{x}{C \setminus x}$. By the triangle inequality and because $x$ is the only point that is close to $C$, we have $L \geq \frac{\delta}{c}$. Define $p_y = \dist{x}{y} / L$ and $p_S = \dist{x}{C \setminus x} / L$ to be the percentage of the distance $L$ from $\dist{x}{y}$ and $\dist{x}{C \setminus x}$ respectively. It is enough for us to show that 

        $$\frac{c}{\lambda}(p_S \cdot L) + \frac{\delta (\lambda - 1)}{(1+c) \lambda} < p_y \cdot L$$

        for all $L \geq \frac{\delta}{c}$. Since this equation is linear in $L$, if it is true for any such $L$ then it is true for $L = \frac{\delta}{c}$. Since $p_y > c \cdot p_S$, we have $p_S < \frac{1}{1 + c}$ and $p_y > \frac{c}{1 + c}$. Plugging in $L = \frac{\delta}{c}$ we get

        \begin{align*}
            \frac{c}{\lambda}\Big(p_S \cdot L\Big) + \frac{\delta (\lambda - 1)}{(1+c) \lambda} &< \frac{c}{\lambda}\Big(\frac{1}{1 + c} \cdot \frac{\delta}{c}\Big) + \frac{\delta (\lambda - 1)}{(1+c) \lambda}\\
            &= \frac{\delta + \delta (\lambda - 1)}{(1+c) \lambda}\\
            &= \frac{\delta}{(1+c)}\\
            &< p_y \cdot \frac{\delta}{c}\\
            &= p_y \cdot L
        \end{align*}

        as desired.
    \end{proof}

%     \wnote{I proved this as if \cref{thm:dynAnn} givs a $c$ approximation and not a $O(c)$ because I'm not completely sure how to handle this.} \enote{By decreasing $c$ by an appropriate constant (hidden in the $O$), you can move the $O$ from the approximation to the runtime.}
% \wnote{Would it make sense to change it in the theorem since that is the form we use or leave it sense that is more common in literature?} \enote{I would leave in more common form}


\hacFinal*

\begin{proof}
    Let $\epsilon = 0.001$ and define $\hat{c} = \frac{c}{1 + \epsilon} > 1.005$. For any $\lambda \in (1,\hat{c})$, \cref{thm:dynAnn} says we can construct a $\Big(\frac{\hat{c}}{\lambda}, \frac{\delta (\lambda - 1)}{(1+\hat{c}) \lambda}\Big)$-approximate nearest neighbor data structure, $\N$, with query, deletion, and amortized insertion time $n^{O(\lambda^2/\hat{c}^2)} \log\Big(\frac{\Delta (1+\hat{c}) \lambda}{\delta (\lambda - 1)}\Big) d^2$. Note that we moved the big $O$ in \cref{thm:dynAnn} from the approximation guarantee to the runtime by scaling by some constant. By \cref{lem:mult_ann}, $\N$ is a $\hat{c}$-approximate ANNS data structure for all queries in \cref{alg:SIMPLE_HAC}. By \cref{thm:general_hac} and our definition of $\hat{c}$, we get $c$-approximate centroid HAC by running \cref{alg:SIMPLE_HAC} with $\N$. The runtime is $\Tilde{O}(n^{1 + O(\lambda^2/\hat{c}^2)} \log\Big(\frac{\Delta (1+\hat{c}) \lambda}{\delta (\lambda - 1)}\Big) d^2)$. Letting $\lambda = 1.005$ and by the assumptions that $\frac{\Delta}{\delta}, c \leq \poly(n)$, all $\log$ terms are dominated by the big $O$ in the exponent and we get the runtime $O(n^{1 + O(1/\hat{c}^2)} d^2) = O(n^{1 + O(1/c^2)} d^2)$.
\end{proof}

In \cref{alg:SIMPLE_HAC}, in the worst case we may have to queue a centroid $\log_{1+\epsilon}(\frac{2 \Delta}{\delta})$ times. However, in practice a centroid may only be queued a small number of times. Say a tuple $(l,x,y)$ in our priority queue becomes stale if the centroid $y$ is merged. Let $\Gamma$ be the average number of tuples in our priority queue that become stale with each merge. Our experiments summarized in \Cref{tab:staleness} suggest that $\Gamma$ is a small constant in practice with $\Gamma < 1$ for all experiments. The following lemma shows that in this case we lose the $\log_{1+\epsilon}(\frac{2 \Delta}{\delta})$ in the runtime.

\begin{lemma}
   If the average number of queued element made stale for each merge in Algorithm \ref{alg:SIMPLE_HAC} is $\Gamma$, then \cref{alg:SIMPLE_HAC} runs in time $O( n \cdot T_I + n \cdot T_D + n \cdot T_Q \cdot \Gamma + n \log (n) \cdot \Gamma)$.
\end{lemma}

\begin{proof}
    There are a total of $n-1$ merges during the runtime of \cref{alg:SIMPLE_HAC} so the total number of tuples that are made stale is $(n - 1) \Gamma$. There are an additional $n-1$ tuples that get merged. Thus, the total number of tuples that get dequeued throughout the runtime of the algorithm is $O(\Gamma)$. The rest of the proof is the same as that of \cref{lem:SIMPLE_HAC_RUNTIME} except we pay the cost of de-queuing on \cref{line:dequeue} $O(n \cdot \Gamma)$ times instead of $n \cdot \log_{1+\epsilon}(\frac{2 \Delta}{\delta})$.
\end{proof}

==> annPseudo.tex <==
\section{Adaptive Dynamic ANN Pseudo-code}\label{sec:annPseudo}

\begin{algorithm}
    \caption{Dynamic ANNS for Adaptive Updates}
    \label{alg:dynANN}
    \begin{algorithmic}[0] % The number tells where the line numbering should start
            \State \textbf{Input:} $\beta$, $\Delta$, $n$, $s \in \mathbb{R}^d$, $Q \gets \textsc{CoveringNet}(s, \Delta, \beta)$ (computed using \Cref{thm:covNet})
            \State \textbf{Maintains:} $S_0, S_1, \ldots$ -- partition of the inserted points, s.t. $|S_i| \leq 2^i$
            \State \textbf{Maintains:} $\N_0, \N_1, \ldots$ -- a non-adaptive ANNS for each $S_i$
           
            \Function{\ANNInsert}{$u$}
            \State $S_0 \gets S_0 \cup \{u\}$
                    
                    \While{$\exists i$ such that $|S_i| > 2^i$} 
                        \State $S_{i+1} \gets S_{i+1} \cup S_i$ and $S_i \gets \emptyset$
                        \State $\N_{i+1} \gets \ANN(S_{i+1})$ and $\N_i \gets \ANN(\emptyset)$
                    \EndWhile
            \EndFunction
          
           \Function{\ANNDelete}{$u$}
                    \State Let $i$ be such that $u \in S_i$
                    \State $\N_i.\ANNDelete(u)$ and remove $u$ from $S_i$
            \EndFunction

             \Function{\ANNQuery}{$u, \bar{u}$}
                    \State Let $u' \in Q$ be such that $\dist{u}{u'} =O(\beta)$ \Comment{computed using \Cref{thm:covNet}} 
                    \State Let $v_i = \N_i.\ANNQuery(u', \bar{u})$
                    \State \Return $v = \argmin_{v_i} \dist{u'}{v_i}$
            \EndFunction
    \end{algorithmic}
\end{algorithm}

==> tables/quality_evals_old.tex <==
\afterpage{\begin{landscape}
\begin{table}
\caption{}
\label{tab:quality-evals-all}
\footnotesize
\begin{tabular}{cccccc|ccccc}
\hline
\multicolumn{1}{l}{} &
  Dataset &
  Centroid\textsubscript{0.1}(H) &
  Centroid\textsubscript{0.2}(H) &
  Centroid\textsubscript{0.4}(H) &
  Centroid\textsubscript{0.8}(H) &
  FC-Centroid &
  FC-Single &
  FC-Complete &
  FC-Avg &
  FC-Ward \\
\hline
\multirow{7}{*}{\begin{sideways}ARI\end{sideways}} & iris   &  \best{0.759} & 0.746 & 0.638 & 0.594 & \best{0.759} & 0.715 & 0.642 & \best{0.759} & 0.731  \\
                     & wine & 0.352 & 0.352 & \best{0.402} & 0.366 & 0.352 & 0.298 & 0.371 & 0.352 & 0.368 \\
                     & cancer & 0.509 & 0.526 & 0.490 & \best{0.641} & 0.509 & 0.561 & 0.465 & 0.537 & 0.406 \\
                     & digits & 0.589 & 0.571 & 0.576 & 0.627 & 0.559 & 0.662 & 0.479 & 0.690 & \best{0.813} \\
                     & faces  & 0.370 & 0.388 & 0.395 & 0.392 & 0.359 & 0.468 & 0.472 & 0.529 & \best{0.608} \\
                     & mnist  &  0.270 & 0.222 & 0.218 & 0.191 & 0.192 & 0.182 & 0.219 & 0.383 & \best{0.544} \\
                     & birds  &  &  &  &  &  &  &  &  &  \\
\hline 
\multirow{7}{*}{\begin{sideways}NMI\end{sideways}} & iris & \best{0.803} & 0.795 & 0.732 & 0.732 & \best{0.803} & 0.732 & 0.718 & \best{0.803} & 0.767 \\
                     & wine   & 0.424 & 0.424 & 0.413 & 0.389 & 0.424 & 0.390 & \best{0.436} & 0.424 & 0.424 \\
                     & cancer & 0.425 & 0.471 & 0.459 & \best{0.528} & 0.425 & 0.249 & 0.425 & 0.454 & 0.421 \\
                     & digits & 0.718 & 0.726 & 0.707 & 0.754 & 0.727 & 0.741 & 0.701 & 0.824 & \best{0.867} \\
                     & faces  & 0.539 & 0.534 & 0.549 & 0.549 & 0.556 & 0.623 & 0.658 & 0.698 & \best{0.746} \\
                     & mnist  &  0.291 & 0.282 & 0.306 & 0.307 & 0.250 & 0.112 & 0.472 & 0.597 & \best{0.697}  \\
                     & birds  &  &  &  &  &  &  &  &  &  \\
\hline
\multirow{7}{*}{\begin{sideways}Purity\end{sideways}} & iris & 0.869 & 0.862 & 0.808 & 0.809 & \best{0.871} & 0.843 & 0.791 & 0.869 & 0.850 \\
                     & wine   & 0.616 & 0.616 & \best{0.640} & 0.601 & 0.616 & 0.584 & 0.607 & 0.620 & 0.616  \\
                     & cancer & 0.816 & 0.818 & 0.805 & 0.836 & 0.816 & 0.798 & 0.804 & \best{0.829} & 0.783  \\
                     & digits & 0.677 & 0.667 & 0.654 & 0.715 & 0.679 & 0.737 & 0.562 & 0.755 & \best{0.851} \\
                     & faces  & 0.460 & 0.477 & 0.478 & 0.488 & 0.467 & 0.566 & 0.502 & \best{0.623} & 0.614 \\
                     & mnist  & 0.310 & 0.286 & 0.283 & 0.278 & 0.308 & 0.238 & 0.301 & 0.511 & \best{0.639} \\
                     & birds  &  &  &  &  &  &  &  &  &  \\
\hline
\multirow{7}{*}{\begin{sideways}Dasgupta\end{sideways}} & iris   &  506011.1 & 506101.2 & 510680.6 & 507149.4 & \best{505809.8} & 519786.5 & 541202.3 & 506091.2 & 508571.4 \\
                     & wine   & 7655.9 & 7655.9 & \best{7545.7} & 7564.2 & 7655.9 & 7815.9 & 7775.0 & 7655.3 & 7558.6  \\
                     & cancer & \best{153644.7} & 153519.2 & 156220.4 & 156893.8 & 153843.2 & 176224.9 & 155255.2 & 154127.1 & 157375.1 \\
                     & digits & 39292919.2 & 39315744.3 & 39299184.6 & 39215081.5 & 39289534.3 & 39732887.1 & 39552462.5 & \best{39009658.8} & 39136177.1 \\
                     & faces  & 1703728.2 & 1703696.7 & 1706886.4 & 1703361.3 & 1704833.1 & 1728503.6 & 1712719.3 & \best{1700185.3} & 1720583.5 \\
                     & mnist  &  &  &  &  &  &  &  &  &  \\
                     & birds  &  &  &  &  &  &  &  &  &  \\
\hline
\end{tabular}
\end{table}
\end{landscape}}
